Vision-Based Perception for Autonomous Vehicles in Off-Road Environment Using Deep Learning

Low-latency intelligent systems are required for autonomous driving on non-uniform terrain in open-pit mines and developing countries. This work proposes a perception system for autonomous vehicles on unpaved roads and off-road environments, capable of navigating rough terrain without a predefined trail. The Configurable Modular Segmentation Network (CMSNet) framework is proposed, facilitating different architectural arrangements. CMSNet configurations were trained to segment obstacles and trafficable ground on new images from unpaved/off-road scenarios with adverse conditions (night, rain, dust). We investigated applying deep learning to detect drivable regions without explicit track boundaries, studied algorithm behavior under visibility impairment, and evaluated field tests with real-time semantic segmentation. A new dataset, Kamino, is presented with almost 12,000 images from an operating vehicle with eight synchronized cameras. The Kamino dataset has a high number of labeled pixels compared to similar public collections and includes images from an off-road proving ground emulating a mine under adverse visibility. To achieve real-time inference, CMSNet CNN layers were methodically removed and fused using TensorRT, C++, and CUDA. Empirical experiments on two datasets validated the proposed system's effectiveness.

==> agradecimentos.tex <==
% ---
% Agradecimentos
% ---
I acknowledge my children, Náthalie and Christian Oliveira Alves, for being my source of inspiration, and my wife, Crisbel Oliveira, who always advised me to move forward. I also acknowledge my mother, Adelaide Maria de Andrade, who always supported me in everything, and my father, Antonio Gilmar Cordeiro Ferreira, my greatest supporter when he was alive.

I acknowledge all the people that directly or indirectly contribute to the realization of this work. Also, the UFBA and PPGEE, especially the advisors, Prof. Dr. Eduardo Furtado de Simas Filho and Prof. Dr. Wagner Luiz Alves de Oliveira, for guiding me on this journey of learning and research. And the SENAI CIMATEC, especially Leonardo Nardy and Marco Reis, for the research support.



==> dedicatoria.tex <==
% ---
% Dedicatória
% ---
I dedicate this work to my wife and children, \\
who supported me during this journey.


==> epigrafe.tex <==
% ---
% Epígrafe
% ---
\aspas{As invenções são, sobretudo, \\
o resultado de um trabalho de teimoso.}\\
		(Santos Dumont)
% ---
